Active Algorithms For Preference Learning Problems with Multiple Populations

In this paper we model the problem of learning preferences of a population as an active learning problem. We propose an algorithm can adaptively choose pairs of items to show to users coming from a heterogeneous population, and use the obtained reward to decide which pair of items to show next. We provide computationally efficient algorithms with provable sample complexity guarantees for this problem in both the noiseless and noisy cases. In the process of establishing sample complexity guarantees for our algorithms, we establish new results using a Nystr{\"o}m-like method which can be of independent interest. We supplement our theoretical results with experimental comparisons.

==> synthetic_results.tex <==
\subsection{Deterministic games on synthetic datasets}
Here we picked the number of arms, $K=400$ and $r=2$. Then we created a random matrix $\mA  \in [0,1]^{K \times r} $. Then taking $\mL = \mA \mA^\top$ gives us a rank $2$ matrix but now its elements might no longer be bounded above by $1$. Therefore dividing $\mA$ by a large enough number such that resultant matrix has entries that represent probabilities gave us the synthetic data to test on. In the case of the approxim ately low-rank matrix, we follow the same steps, except that we added to $\mA$ a perturbation matrix $\epsilon \mE, \epsilon = 10^{-4}, \mE \in [0,1]^{K \times r}$. We also ensured that the minimum of the matrix occurred on an off-diagonal element in order to ensure that the results would be non-trivial.
\subsection*{Noiseless results}
The results can be seen in tables \ref{tab:exactranknonoise} and \ref{tab:approxranknonoise}. Notice that the number of samples for the Naive algorithm doesn't change as in the noiseless case, it always samples all ${K \choose r}$ arms. As it can be seen, our algorithm out performs the other algorithms by a considerable margin.

\begin{table}
\centering
    \caption{Comparison of results for the low rank case with exact rank, where we have 400 arms. }
    \begin{tabular}{| l | l | l |}
    \hline
    Algorithm & Samples (rank 2) & Samples (rank 100) \\ \hline
    Naive & 79800 & 79800  \\      \hline
    Nystr{\"o}m & 8000 & 4240000  \\ \hline
    MISA & 1197 & 1197 \\ \hline
    \end{tabular}
    \label{tab:exactranknonoise}
\end{table}

\begin{table}
\centering
    \caption{Comparison of results for the low rank case with approximate rank, where we have 400 arms.}
    \begin{tabular}{| l | l | l |}
    \hline
    Algorithm & Samples (rank 2) & Samples (rank 100) \\ \hline
    Naive & 79800 & 79800 \\      \hline
    Nystr{\"o}m & 8000 & 1844000  \\ \hline
    MISA & 1594 & 11194 \\ \hline
    \end{tabular}
    \label{tab:approxranknonoise}
\end{table}
